Classification, Challenges, and Automated Approaches to Handle Non-Functional Requirements in ML-Enabled Systems: A Systematic Literature Review

Context: Machine learning (ML) is nowadays so pervasive and diffused that virtually no application can avoid its use. Nonetheless, its enormous potential is often tempered by the need to manage non-functional requirements and navigate pressing, contrasting trade-offs. Objective: In this respect, we notice the lack of a comprehensive synthesis of the non-functional requirements affecting ML-enabled systems, other than the major challenges faced to deal with them. Such a synthesis may not only provide a comprehensive summary of the state of the art, but also drive further research on the analysis, management, and optimization of non-functional requirements of ML-intensive systems. Method: In this paper, we propose a systematic literature review targeting two key aspects such as (1) the classification of the non-functional requirements investigated so far, and (2) the challenges to be faced when developing models in ML-enabled systems. Through the combination of well-established guidelines for conducting systematic literature reviews and additional search criteria, we survey a total amount of 69 research articles. Results: Our findings report that current research identified 30 different non-functional requirements, which can be grouped into six main classes. We also compiled a catalog of more than 23 software engineering challenges, based on which further research should consider the nonfunctional requirements of machine learning-enabled systems. Conclusion: We conclude our work by distilling implications and a future outlook on the topic.

==> author.tex <==
\author{Vincenzo De Martino}
\email{vdemartino@unisa.it}
\affiliation{%
  \institution{SeSa Lab -- University of Salerno}
  \city{Salerno}
  \country{Italy}
}

\author{Fabio Palomba}
\email{fpalomba@unisa.it}
\affiliation{%
  \institution{SeSa Lab -- University of Salerno}
  \city{Salerno}
  \country{Italy}
}

==> sd.tex <==
\begin{table}
    \centering
    \caption{Identified Best Practices for \textbf{Bots Interaction and Adoption}.}
    \vspace{1mm} % Adjust the height of the space between caption and tabular
    
    \rowcolors{1}{graytable}{white}
    \resizebox{\linewidth}{!}{
\begin{tabular}{lrlrrllllrlrlllllll}
\rowcolor[HTML]{000000} 
{\color[HTML]{FFFFFF} }                                                                                                          & {\color[HTML]{FFFFFF} \textbf{Interruption and Noise}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Long Response Latency}}} & {\color[HTML]{FFFFFF} \textbf{Contextual Information}} & {\color[HTML]{FFFFFF} \textbf{Usability}}    & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{NLP and NLU}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Uncanny Valley}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Malicious Intent}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Bias Information}}} & {\color[HTML]{FFFFFF} \textbf{Motivation}}   & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Discoverability}}} & {\color[HTML]{FFFFFF} \textbf{Trust}}        & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Terms of Serveice}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Configuration and Customization}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Framework}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Testing}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Maintenance}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Architecture}}} & \multicolumn{1}{p}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Integration}}} \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Implement a System to evaluate bot choices}}                               & 1                                                      &                                                                                                   & 1                                                      & 1                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 1                                            &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                            &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Follow a modular architecture}}                                            & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                                     & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & 1                                            & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                           &                                                                                            &                                                                                              &                                                                                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                               &                                                                                                             &                                                                                       & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                       & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                           & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}2}                                            &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Make bots adaptive and able to learn over time using AI}}                  & 1                                                      & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                                     & 2                                                      & 2                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 1                                            &                                                                                             & 2                                            &                                                                                               &                                                                                                             &                                                                                       & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                       &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}2}                                            &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Adopt a specific lifecycle process for bots}}                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                         &                                                                                            &                                                                                              &                                                                                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Carefully select the correct framework based on bot requirements}}         & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                         &                                                                                            &                                                                                              &                                                                                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                               &                                                                                                             & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}4}                                         &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Integrate bots actions in a way that do not interrupt developer workflow}} & 1                                                      &                                                                                                   & 1                                                      & 2                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 2                                            &                                                                                             & 3                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Allow developers to edit bot configuration easily}}                        & 1                                                      &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & 1                                            & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                           &                                                                                            &                                                                                              &                                                                                              & 1                                            &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Provide bot with personality}}                                             & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & 1                                            &                                                                                         &                                                                                            &                                                                                              &                                                                                              & 1                                            &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Design a Smooth and frictionless interaction}}                             & 2                                                      &                                                                                                   & 2                                                      & 2                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 1                                            &                                                                                             & 2                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Enforce transparency in bot actions and outputs}}                          & 2                                                      &                                                                                                   & 1                                                      & 1                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 2                                            &                                                                                             & 2                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Integrating concepts from behavioral science in interaction flow}}         & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           &                                                                                                   & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}}           & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                         &                                                                                            &                                                                                              &                                                                                              & \multicolumn{1}{l}{\cellcolor[HTML]{FFFFFF}} &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                            &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Provide users with a high level of control over bot}}                      & 2                                                      &                                                                                                   & 3                                                      & 3                                            &                                                                                         & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                              &                                                                                              &                                                                                              & 2                                            &                                                                                             & 3                                            &                                                                                               &                                                                                                             &                                                                                       &                                                                                     &                                                                                         &                                                                                          &                                                                                         \\
\rowcolor[HTML]{FFFFFF} 
\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Create a reliable test infrastructure}}                                    & 1                                                      & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                                     & 1                                                      & 1                                            &                                                                                         &                                                                                            &                                                                                              &                                                                                              & 1                                            &                                                                                             & 1                                            &                                                                                               &                                                                                                             &                                                                                       & \multicolumn{1}{p}{\cellcolor[HTML]{FFFFFF}1}                                       &                                                                                         &                                                                                          &                                                                                        
\end{tabular}
}
    
    \label{table:best_practices_interaction}
\end{table}

==> sections/old_table_discussion.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
%\begin{landscape}
\begin{table}[]
\centering
% Adjust the height of the space between caption and tabular

\resizebox{\linewidth}{!}{%
\begin{tabular}{|
>{\columncolor[HTML]{000000}}p{0.3\linewidth} |
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |}
\toprule
\multicolumn{1}{|c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} }} &
  \multicolumn{8}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Challenges - Part 1}}} \\ \cline{2-9} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Best Practices}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Interruption and Noise}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Long Response Latency}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Contextual Information}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Usability}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{NLP and NLU}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Uncanny Valley}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Malicious Intent}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Bias Information}}}} \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Implement a System to evaluate bot choices}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Follow a modular architecture}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Make bots adaptive and able to learn over time using AI}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Adopt a specific lifecycle process for bots}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Carefully select the correct framework based on bot requirements}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Integrate bots actions in a way that do not interrupt developer workflow}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Allow developers to edit bot configuration easily}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Provide bot with personality}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Design a Smooth and frictionless interaction}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Enforce transparency in bot actions and outputs}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Integrating concepts from behavioral science in interaction flow}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Provide users with a high level of control over bot}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Create a reliable test infrastructure}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
   \bottomrule
\end{tabular}%
}
\label{table:cahllenge_best_practices_1}
\end{table}

\begin{table}[]
    \centering
\caption{Match between best practices and challenges - Part 2.}
\vspace{1mm} % Adjust the height of the space between caption and tabular

\resizebox{\linewidth}{!}{%
    \begin{tabular}{|
>{\columncolor[HTML]{000000}}p{0.3\linewidth} |
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}r 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l 
>{\columncolor[HTML]{FFFFFF}}l |}
\toprule
\multicolumn{1}{|c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} }} &
  \multicolumn{10}{c|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Challenges - Part 2}}} \\ \cline{2-11} 
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textbf{Best Practices}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Motivation}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Discoverability}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Trust}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Terms of Serveice}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Configuration and Customization}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Framework}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Testing}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Maintenance}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Architecture}}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{000000}{\color[HTML]{FFFFFF} \textit{\textbf{Integration}}}} \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Implement a System to evaluate bot choices}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Follow a modular architecture}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Make bots adaptive and able to learn over time using AI}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Adopt a specific lifecycle process for bots}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Carefully select the correct framework based on bot requirements}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}4} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Integrate bots actions in a way that do not interrupt developer workflow}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Allow developers to edit bot configuration easily}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Provide bot with personality}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Design a Smooth and frictionless interaction}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Enforce transparency in bot actions and outputs}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Integrating concepts from behavioral science in interaction flow}}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Provide users with a high level of control over bot}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}2} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}3} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
{\color[HTML]{FFFFFF} \textit{\textbf{Create a reliable test infrastructure}}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{r|}{\cellcolor[HTML]{FFFFFF}1} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
  \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}} &
   \\ \hline
   \bottomrule
\end{tabular}%
}
    \label{table:cahllenge_best_practices_2}
\end{table}

